Multilingual Code Co-Evolution Using Large Language Models

Many software projects implement APIs and algorithms in multiple programming languages. Maintaining such projects is tiresome, as developers have to ensure that any change (e.g., a bug fix or a new feature) is being propagated, timely and without errors, to implementations in other programming languages. In the world of ever-changing software, using rule-based translation tools (i.e., transpilers) or machine learning models for translating code from one language to another provides limited value. Translating each time the entire codebase from one language to another is not the way developers work. In this paper, we target a novel task: translating code changes from one programming language to another using large language models (LLMs). We design and implement the first LLM, dubbed Codeditor, to tackle this task. Codeditor explicitly models code changes as edit sequences and learns to correlate changes across programming languages. To evaluate Codeditor, we collect a corpus of 6,613 aligned code changes from 8 pairs of open-source software projects implementing similar functionalities in two programming languages (Java and C#). Results show that Codeditor outperforms the state-of-the-art approaches by a large margin on all commonly used automatic metrics. Our work also reveals that Codeditor is complementary to the existing generation-based models, and their combination ensures even greater performance.

==> figures/defs-code.tex <==
%%% defs-code.tex
%%% Utility Commands for Code Listings
%%% Version 1.0.2

%%%==========
%%% COPIED FROM vkuncak/doc/vmcai09/defs.tex
\definecolor{gray}{RGB}{211,211,211}
\definecolor{javared}{rgb}{0.6,0,0} % for strings
\definecolor{javagreen}{rgb}{0.25,0.5,0.35} % comments
\definecolor{javapurple}{rgb}{0.5,0,0.2} % keywords
\definecolor{javadocblue}{rgb}{0.25,0.35,0.75} % javadoc
\newcommand{\jbasicstyle}{\small\sffamily} % Style of code
\newcommand{\textcode}[1]{{#1}}
\newcommand{\jnumberstyle}{\scriptsize}
\newcommand{\Hilight}{\makebox[0pt][l]{\color{gray}\rule[-3pt]{0.80\linewidth}{9pt}}}

\lstdefinelanguage{pseudo}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=left, % none for no numbers
  numberstyle=\jnumberstyle,
  numbersep=4pt,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=10pt,
%  mathescape=false,
}

\lstdefinelanguage{todo-comment}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=none,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=-10pt,
%  mathescape=false,
}

\lstdefinelanguage{java-pretty}
{
  language=java,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  columns=fullflexible,
  % xleftmargin=20pt,
  showstringspaces=false,
  keywordstyle=\bfseries\color{javadocblue},
  stringstyle=\color{javared},
  commentstyle=\color{javagreen},
  numbersep=-12pt,
  morecomment=[s][\color{javadocblue}]{/**}{*/},
  moredelim=[is][\color{red!50!black}]{(-W<)}{(>W-)},
  moredelim=[is][\bfseries\color{red!80!black}]{(-w<)}{(>w-)},
  moredelim=[is][\color{green!30!black}]{(+W<)}{(>W+)},
  moredelim=[is][\bfseries\color{green!60!black}]{(+w<)}{(>w+)},
}



\lstset{escapeinside={(*@}{@*)}}

%%%==========


==> figures/defs-logic.tex <==
%%% defs-logic.tex
%%% Utility Commands for Logic Symbols
%%% Version 1.1.0

%%% Basic Logic
% True & False
\newcommand{\ltrue}{\top} % ⊤
\newcommand{\lfalse}{\bot} % ⊥

% Operators
% \land ∧
% \lor ∨
% \lnot ¬
\newcommand{\limply}{\rightarrow} % →
\newcommand{\liff}{\leftrightarrow} % ↔
\newcommand{\lcofactor}{\downarrow} % ↓

\newcommand{\llimply}{\Rightarrow} % ⇒
\newcommand{\lliff}{\Leftrightarrow} % ⇔
\newcommand{\lsat}{\vDash} % ⊨
\newcommand{\lnsat}{\nvDash} % ⊭

% Quantifiers
\newcommand{\lqall}[1]{\forall #1.~} % ∀x.
\newcommand{\lqexist}[1]{\exists #1.~} % ∃x.
\newcommand{\lqallOnly}[1]{\forall #1 } % ∀x
\newcommand{\lqexistOnly}[1]{\exists #1 } % ∃x

% Big Operators
\newcommand{\lAnd}[1]{\bigwedge_{\substack{#1}}} % ⋀
\newcommand{\lOr}[1]{\bigvee_{\substack{#1}}} % ⋁

%%% Set
\newcommand{\set}[1]{\{#1\}} % {x, y, z}
\newcommand{\Set}[1]{\left\{#1\right\}} % \left{ x, y, z \right}
\newcommand{\tuple}[1]{\langle#1\rangle} % <a, b, c>
\newcommand{\Tuple}[1]{\left\langle#1\right\rangle} % \left< a, b, c \right>

\newcommand{\sunion}{\cup} % ∪
\newcommand{\sinter}{\cap} % ∩


==> figures/intro-example-old.tex <==

\newsavebox\boxCsMethod
\begin{lrbox}{\boxCsMethod}
  \begin{lstlisting}[language=java-pretty]
    [NUnit.Framework.Test] 
    public virtual void Equality() {
      Tag p1 = Tag.ValueOf("p");
      Tag p2 = Tag.ValueOf("p");
      NUnit.Framework.Assert.(-W<)IsTrue(p1.Equals(p2))(>W-);
      NUnit.Framework.Assert.(-W<)IsTrue(p1 == p2)(>W-);
    }

    [NUnit.Framework.Test] 
    public virtual void Equality() {
      Tag p1 = Tag.ValueOf("p");
      Tag p2 = Tag.ValueOf("p");
      NUnit.Framework.Assert.(+W<)AreEqual(p1, p2)(>W+);
      NUnit.Framework.Assert.(+W<)AreSame(p1, p2)(>W+);
    }
  \end{lstlisting}
\end{lrbox}

\newsavebox\boxJavaMethod
\begin{lrbox}{\boxJavaMethod}
  \begin{lstlisting}[language=java-pretty]
    @Test 
    public void equality() {
      Tag p1 = Tag.valueOf("p");
      Tag p2 = Tag.valueOf("p");
      (-W<)assertTrue(p1.equals(p2))(>W-);
      (-W<)assertTrue(p1 == p2)(>W-);
    }

    @Test 
    public void equality() {
      Tag p1 = Tag.valueOf("p");
      Tag p2 = Tag.valueOf("p");
      (+W<)assertEquals(p1, p2)(>W+);
      (+W<)assertSame(p1, p2)(>W+);
    }
  \end{lstlisting}
\end{lrbox}


\begin{tikzpicture}[
    line width=0.4pt,
    node distance=0ex and 0em,
    every node/.style={scale=1},
    gridBox/.style={rectangle, opacity=0, draw=red},
    box/.style={rectangle, draw=black, inner sep=2pt, font=\small},
    rounded box/.style={rectangle, rounded corners, draw=black, inner sep=2pt, font=\small},
    anno/.style={font=\footnotesize},
]

    \DefMacro{wCodeBox}{25em}
    \DefMacro{hCodeBox}{32ex}
    
    \node (g-Old) at (0,0) [box, minimum width=\UseMacro{wCodeBox}, minimum height=\UseMacro{hCodeBox}] {};
    \node (b-Old) [right = -0.3 of g-Old.west] [] {\usebox\boxJavaMethod};
    \node (b-OldText) [below left = 1pt and 1pt of g-Old.north east] [box, draw=red!50, fill=red!20, scale=0.8] {\bf Java Old\phantom{p\hskip -.6em}};
    \node (b-OldText) [below left = 60pt and 1pt of g-Old.north east] [box, draw=green!50, fill=green!20, scale=0.8] {\bf Java New\phantom{p\hskip -.6em}};
    \node (g-New) [below = 0 of g-Old.south] [box, minimum width=\UseMacro{wCodeBox}, minimum height=\UseMacro{hCodeBox}] {};
    \node (b-New) [right = -0.3 of g-New.west] [] {\usebox\boxCsMethod};
    \node (b-NewText) [below left = 1pt and 1pt of g-New.north east] [box, draw=red!50, fill=red!20, scale=0.8] {\bf C\# Old};
    \node (b-NewText) [below left = 60pt and 1pt of g-New.north east] [box, draw=green!50, fill=green!20, scale=0.8] {\bf C\# New\phantom{p\hskip -.6em}};
    
\end{tikzpicture}

==> figures/model-architecture.tex <==
% Define block styles
\tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=2.5cm,minimum height=2em]
\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110,minimum height=2em,text centered, draw=black, fill=blue!30]
\tikzstyle{model} = [rectangle, draw, text width=10em, text badly centered, minimum height=2em, node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, text width=10em, rounded corners, minimum height=2em]
  \tikzstyle{line} = [draw, -latex']
\begin{tikzpicture}[node distance = 1.5cm, auto]
    % Place nodes
    % \node [io] (init) {Initialize};
    % \node [cloud, above of=init] (Start) {Start};
    % \node [cloud, right of=init] (system) {system};
    \node [block] (javaEdits) {\texttt{\tiny<ReplaceOld> long <ReplaceNew> public long <ReplaceEnd>}};
    \node [block, below of=javaEdits] (csOld) {\tiny\texttt{internal virtual long LastModified() \dots}};
    \node [block, below of=csOld] (javaNew) {\tiny\texttt{internal virtual long LastModified() \dots} };
    \node[model, right of=csOld, node distance=5cm] (deltaModel) {\DeltaTool};
    \node [block, right of=deltaModel, node distance=5cm] (csEdits) {\texttt{\tiny<ReplaceOld> internal <ReplaceNew> public <ReplaceEnd>}};
    \node [block, below of=csEdits,] (csCode) {\texttt{\tiny public virtual long LastModified() ...}};
    % \node [decision, below of=evaluate] (decide) {Decision};
    % \node [cloud, below of=decide, node distance=3cm] (Stop) {Stop};
    % % Draw edges
    \path [line] (javaEdits) -- (deltaModel);
    \path [line] (csOld) -- (deltaModel);
    \path [line] (javaNew) -- (deltaModel);
    \path [line] (deltaModel) -- (csEdits);
    \path [line] (csEdits) -- (csCode);
    % \path [line] (decide) -- node {no}(Stop);
    % \path [line,dashed] (Start) -- (init);
    % \path [line,dashed] (system) -- (init);
    % \path [line,dashed] (system) |- (evaluate);
\end{tikzpicture}

==> tables/numbers-java2cs-clean-translation-models-results.tex <==

%% Automatically generated by pyutil.latex 

\DefMacro{res-java2cs-clean-translation-CodeT5-Acc-top-1}{49.50}
\DefMacro{res-java2cs-clean-translation-CodeT5-BLEU}{90.84}
\DefMacro{res-java2cs-clean-translation-CodeT5-COPY-PCT}{0.00}
\DefMacro{res-java2cs-clean-translation-CodeT5-CodeBLEU}{82.37}
\DefMacro{res-java2cs-clean-translation-CodeT5-ag-Acc-top-1}{52.48}
\DefMacro{res-java2cs-clean-translation-CodeT5-ag-BLEU}{91.12}
\DefMacro{res-java2cs-clean-translation-CodeT5-ag-COPY-PCT}{0.00}
\DefMacro{res-java2cs-clean-translation-CodeT5-ag-CodeBLEU}{84.30}
\DefMacro{res-java2cs-clean-translation-CoditT5-Acc-top-1}{23.60}
\DefMacro{res-java2cs-clean-translation-CoditT5-BLEU}{69.83}
\DefMacro{res-java2cs-clean-translation-CoditT5-COPY-PCT}{0.00}
\DefMacro{res-java2cs-clean-translation-CoditT5-CodeBLEU}{61.16}
\DefMacro{res-java2cs-clean-update-CodeT5-Acc-top-1}{57.43}
\DefMacro{res-java2cs-clean-update-CodeT5-BLEU}{93.37}
\DefMacro{res-java2cs-clean-update-CodeT5-COPY-PCT}{0.00}
\DefMacro{res-java2cs-clean-update-CodeT5-CodeBLEU}{87.57}
\DefMacro{res-java2cs-clean-update-CodeT5-ag-Acc-top-1}{71.91}
\DefMacro{res-java2cs-clean-update-CodeT5-ag-BLEU}{97.30}
\DefMacro{res-java2cs-clean-update-CodeT5-ag-COPY-PCT}{10.11}
\DefMacro{res-java2cs-clean-update-CodeT5-ag-CodeBLEU}{94.55}
\DefMacro{res-java2cs-clean-align-CoditT5-Acc-top-1}{68.54}
\DefMacro{res-java2cs-clean-align-CoditT5-BLEU}{95.93}
\DefMacro{res-java2cs-clean-align-CoditT5-COPY-PCT}{10.67}
\DefMacro{res-java2cs-clean-align-CoditT5-CodeBLEU}{92.80}
\DefMacro{res-java2cs-clean-align-CoditT5-ag-Acc-top-1}{67.98}
\DefMacro{res-java2cs-clean-align-CoditT5-ag-BLEU}{95.06}
\DefMacro{res-java2cs-clean-align-CoditT5-ag-COPY-PCT}{14.61}
\DefMacro{res-java2cs-clean-align-CoditT5-ag-CodeBLEU}{91.75}


==> tables/table-clean-test-java2cs-translation-models-results.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}[t]
\begin{center}
\caption{\UseMacro{TCap-clean-test-java2cs-translation-models-results}}
\begin{tabular}{l | c  c  c  c }
\toprule
\textbf{\UseMacro{THead-models}}
 & \textbf{\UseMacro{THead-Acc-top-1}}
 & \textbf{\UseMacro{THead-BLEU}}
 & \textbf{\UseMacro{THead-CodeBLEU}}
\\
\midrule
\UseMacro{THead-translation-CodeT5}
 & \UseMacro{res-clean-test-java2cs-translation-CodeT5-Acc-top-1}$^{\chi}$
 & \UseMacro{res-clean-test-java2cs-translation-CodeT5-BLEU}
 & \UseMacro{res-clean-test-java2cs-translation-CodeT5-CodeBLEU}
\\
\UseMacro{THead-translation-CodeT5-ag}
 & \UseMacro{res-clean-test-java2cs-translation-CodeT5-ag-Acc-top-1}
 & \UseMacro{res-clean-test-java2cs-translation-CodeT5-ag-BLEU}
 & \UseMacro{res-clean-test-java2cs-translation-CodeT5-ag-CodeBLEU}
\\
\UseMacro{THead-translation-CoditT5}
 & \UseMacro{res-clean-test-java2cs-translation-CoditT5-Acc-top-1}$^{\chi}$
 & \UseMacro{res-clean-test-java2cs-translation-CoditT5-BLEU}
 & \UseMacro{res-clean-test-java2cs-translation-CoditT5-CodeBLEU}
\\
\UseMacro{THead-update-CodeT5}
 & \UseMacro{res-clean-test-java2cs-update-CodeT5-Acc-top-1}
 & \UseMacro{res-clean-test-java2cs-update-CodeT5-BLEU}
 & \UseMacro{res-clean-test-java2cs-update-CodeT5-CodeBLEU}
\\
\UseMacro{THead-update-CodeT5-ag}
 & \textbf{\UseMacro{res-clean-test-java2cs-update-CodeT5-ag-Acc-top-1}}
 & \textbf{\UseMacro{res-clean-test-java2cs-update-CodeT5-ag-BLEU}}
 & \textbf{\UseMacro{res-clean-test-java2cs-update-CodeT5-ag-CodeBLEU}}
\\
\UseMacro{THead-CoditT5}
 & \UseMacro{res-clean-test-java2cs-CoditT5-Acc-top-1}
 & \UseMacro{res-clean-test-java2cs-CoditT5-BLEU}$^{\alpha}$
 & \UseMacro{res-clean-test-java2cs-CoditT5-CodeBLEU}$^{\beta}$
\\
\UseMacro{THead-CoditT5-ag}
 & \UseMacro{res-clean-test-java2cs-CoditT5-ag-Acc-top-1}
 & \UseMacro{res-clean-test-java2cs-CoditT5-ag-BLEU}$^{\alpha}$
 & \UseMacro{res-clean-test-java2cs-CoditT5-ag-CodeBLEU}$^{\beta}$
\\
\UseMacro{THead-copy}
 & \UseMacro{res-clean-test-java2cs-copy-Acc-top-1}
 & \UseMacro{res-clean-test-java2cs-copy-BLEU}
 & \UseMacro{res-clean-test-java2cs-copy-CodeBLEU}
\\
\bottomrule
\end{tabular}
\label{tab:clean-test-java2cstranslation-results}
\end{center}
\end{table*}


==> tables/table-cs2java-cp-translation-models-results.tex <==
%% Automatically generated by: Table.py make_table_results

\begin{table*}[t]
\begin{center}
\caption{\UseMacro{TCap-cs2java-cp-translation-models-results}}
\vspace{-8pt}
\begin{tabular}{l | c  c  c  c  c  c }
\toprule
\textbf{\UseMacro{THead-models}}
 & \textbf{\UseMacro{THead-Acc-top-1}}
 & \textbf{\UseMacro{THead-BLEU}}
 & \textbf{\UseMacro{THead-CodeBLEU}}
 & \textbf{\UseMacro{THead-SARI}}
 & \textbf{\UseMacro{THead-GLEU}}
\\
\midrule
\UseMacro{THead-copy}
 & \UseMacro{res-cs2java-cp-copy-Acc-top-1}
 & \UseMacro{res-cs2java-cp-copy-BLEU}
 & \UseMacro{res-cs2java-cp-copy-CodeBLEU}
 & \UseMacro{res-cs2java-cp-copy-SARI}
 & \UseMacro{res-cs2java-cp-copy-GLEU}
\\
\UseMacro{THead-CopyEdits}
 & \UseMacro{res-cs2java-cp-CopyEdits-Acc-top-1}
 & \UseMacro{res-cs2java-cp-CopyEdits-BLEU}
 & \UseMacro{res-cs2java-cp-CopyEdits-CodeBLEU}
 & \UseMacro{res-cs2java-cp-CopyEdits-SARI}
 & \UseMacro{res-cs2java-cp-CopyEdits-GLEU}
\\
\midrule
\UseMacro{THead-translation-CodeT5}
 & \UseMacro{res-cs2java-cp-translation-CodeT5-Acc-top-1}
 & \UseMacro{res-cs2java-cp-translation-CodeT5-BLEU}
 & \UseMacro{res-cs2java-cp-translation-CodeT5-CodeBLEU}
 & \UseMacro{res-cs2java-cp-translation-CodeT5-SARI}
 & \UseMacro{res-cs2java-cp-translation-CodeT5-GLEU}
\\
\UseMacro{THead-update-CodeT5}
 & \UseMacro{res-cs2java-cp-update-CodeT5-Acc-top-1}
 & \UseMacro{res-cs2java-cp-update-CodeT5-BLEU}
 & \UseMacro{res-cs2java-cp-update-CodeT5-CodeBLEU}
 & \UseMacro{res-cs2java-cp-update-CodeT5-SARI}
 & \UseMacro{res-cs2java-cp-update-CodeT5-GLEU}
\\
\UseMacro{THead-CoditT5}
 & \UseMacro{res-cs2java-cp-CoditT5-Acc-top-1}
 & \UseMacro{res-cs2java-cp-CoditT5-BLEU}
 & \UseMacro{res-cs2java-cp-CoditT5-CodeBLEU}
 & \UseMacro{res-cs2java-cp-CoditT5-SARI}
 & \UseMacro{res-cs2java-cp-CoditT5-GLEU}
\\
\UseMacro{THead-chatgpt3.5-zero-shot}
 & \UseMacro{res-cs2java-cp-chatgpt3.5-zero-shot-Acc-top-1}
 & \UseMacro{res-cs2java-cp-chatgpt3.5-zero-shot-BLEU}
 & \UseMacro{res-cs2java-cp-chatgpt3.5-zero-shot-CodeBLEU}
 & \UseMacro{res-cs2java-cp-chatgpt3.5-zero-shot-SARI}
 & \UseMacro{res-cs2java-cp-chatgpt3.5-zero-shot-GLEU}
\\
\midrule
\UseMacro{THead-metaEdits}
 & \UseMacro{res-cs2java-cp-metaEdits-Acc-top-1}
 & \UseMacro{res-cs2java-cp-metaEdits-BLEU}$^{\alpha}$
 & \UseMacro{res-cs2java-cp-metaEdits-CodeBLEU}
 & \UseMacro{res-cs2java-cp-metaEdits-SARI}
 & \UseMacro{res-cs2java-cp-metaEdits-GLEU}$^{\beta}$
\\
\UseMacro{THead-edit-translation}
 & \UseMacro{res-cs2java-cp-edit-translation-Acc-top-1}
 & \UseMacro{res-cs2java-cp-edit-translation-BLEU}$^{\alpha}$
 & \UseMacro{res-cs2java-cp-edit-translation-CodeBLEU}
 & \UseMacro{res-cs2java-cp-edit-translation-SARI}
 & \UseMacro{res-cs2java-cp-edit-translation-GLEU}$^{\beta}$
\\
\midrule
\UseMacro{THead-hybrid}
 & \textbf{\UseMacro{res-cs2java-cp-hybrid-Acc-top-1}}
 & \textbf{\UseMacro{res-cs2java-cp-hybrid-BLEU}}
 & \textbf{\UseMacro{res-cs2java-cp-hybrid-CodeBLEU}}
 & \textbf{\UseMacro{res-cs2java-cp-hybrid-SARI}}
 & \textbf{\UseMacro{res-cs2java-cp-hybrid-GLEU}}
\\
\bottomrule
\end{tabular}
\label{tab:cs2java-cp-translation-results}
\end{center}
\end{table*}

==> tables/table-cs2java-translation-models-results.tex <==
%% Automatically generated by: Table.py make_table_results

\begin{table*}[t]
\begin{center}
\caption{\UseMacro{TCap-cs2java-translation-models-results}}
\vspace{-8pt}
\begin{tabular}{l | c  c  c  c  c  c }
\toprule
\textbf{\UseMacro{THead-models}}
 & \textbf{\UseMacro{THead-Acc-top-1}}
 & \textbf{\UseMacro{THead-BLEU}}
 & \textbf{\UseMacro{THead-CodeBLEU}}
 & \textbf{\UseMacro{THead-SARI}}
 & \textbf{\UseMacro{THead-GLEU}}
\\
\midrule
\UseMacro{THead-copy}
 & \UseMacro{res-cs2java-copy-Acc-top-1}
 & \UseMacro{res-cs2java-copy-BLEU}
 & \UseMacro{res-cs2java-copy-CodeBLEU}
 & \UseMacro{res-cs2java-copy-SARI}
 & \UseMacro{res-cs2java-copy-GLEU}
\\
\UseMacro{THead-CopyEdits}
 & \UseMacro{res-cs2java-CopyEdits-Acc-top-1}
 & \UseMacro{res-cs2java-CopyEdits-BLEU}$^{\alpha}$
 & \UseMacro{res-cs2java-CopyEdits-CodeBLEU}$^{\beta}$
 & \UseMacro{res-cs2java-CopyEdits-SARI}
 & \UseMacro{res-cs2java-CopyEdits-GLEU}$^{\chi}$
\\
\midrule
\UseMacro{THead-translation-CodeT5}
 & \UseMacro{res-cs2java-translation-CodeT5-Acc-top-1}
 & \UseMacro{res-cs2java-translation-CodeT5-BLEU}$^{\alpha}$
 & \UseMacro{res-cs2java-translation-CodeT5-CodeBLEU}$^{\beta}$
 & \UseMacro{res-cs2java-translation-CodeT5-SARI}
 & \UseMacro{res-cs2java-translation-CodeT5-GLEU}$^{\chi}$
\\
\UseMacro{THead-update-CodeT5}
 & \UseMacro{res-cs2java-update-CodeT5-Acc-top-1}
 & \UseMacro{res-cs2java-update-CodeT5-BLEU}
 & \UseMacro{res-cs2java-update-CodeT5-CodeBLEU}$^{\gamma}$
 & \UseMacro{res-cs2java-update-CodeT5-SARI}
 & \UseMacro{res-cs2java-update-CodeT5-GLEU}
\\
\UseMacro{THead-CoditT5}
 & \UseMacro{res-cs2java-CoditT5-Acc-top-1}
 & \UseMacro{res-cs2java-CoditT5-BLEU}
 & \UseMacro{res-cs2java-CoditT5-CodeBLEU}$^{\gamma}$
 & \UseMacro{res-cs2java-CoditT5-SARI}
 & \UseMacro{res-cs2java-CoditT5-GLEU}
\\
\UseMacro{THead-codex}
 & \UseMacro{res-cs2java-codex-Acc-top-1}
 & \UseMacro{res-cs2java-codex-BLEU}
 & \UseMacro{res-cs2java-codex-CodeBLEU}
 & \UseMacro{res-cs2java-codex-SARI}
 & \UseMacro{res-cs2java-codex-GLEU}
\\
\UseMacro{THead-chatgpt3.5-zero-shot}
 & \UseMacro{res-cs2java-chatgpt3.5-zero-shot-Acc-top-1}
 & \UseMacro{res-cs2java-chatgpt3.5-zero-shot-BLEU}
 & \UseMacro{res-cs2java-chatgpt3.5-zero-shot-CodeBLEU}
 & \UseMacro{res-cs2java-chatgpt3.5-zero-shot-SARI}
 & \UseMacro{res-cs2java-chatgpt3.5-zero-shot-GLEU}
\\
\midrule
\UseMacro{THead-metaEdits}
 & \textbf{\UseMacro{res-cs2java-metaEdits-Acc-top-1}}$^{\epsilon}$$^{\eta}$
 & \UseMacro{res-cs2java-metaEdits-BLEU}
 & \UseMacro{res-cs2java-metaEdits-CodeBLEU}
 & \UseMacro{res-cs2java-metaEdits-SARI}
 & \UseMacro{res-cs2java-metaEdits-GLEU}
\\
\UseMacro{THead-edit-translation}
 & \UseMacro{res-cs2java-edit-translation-Acc-top-1}$^{\delta}$$^{\epsilon}$
 & \UseMacro{res-cs2java-edit-translation-BLEU}
 & \UseMacro{res-cs2java-edit-translation-CodeBLEU}
 & \textbf{\UseMacro{res-cs2java-edit-translation-SARI}}
 & \UseMacro{res-cs2java-edit-translation-GLEU}
\\
\midrule
\UseMacro{THead-hybrid}
 & \UseMacro{res-cs2java-hybrid-Acc-top-1}$^{\delta}$$^{\eta}$
 & \textbf{\UseMacro{res-cs2java-hybrid-BLEU}}
 & \textbf{\UseMacro{res-cs2java-hybrid-CodeBLEU}}
 & \UseMacro{res-cs2java-hybrid-SARI}
 & \textbf{\UseMacro{res-cs2java-hybrid-GLEU}}
\\
\bottomrule
\end{tabular}
\vspace{\UseMacro{TVspace-cs2java-translation-models-results}}
\end{center}
\end{table*}

==> tables/table-dataset-edits-stats.tex <==

%% Automatically generated by pyutil.latex 
%% manually tuned by Jiyang

\begin{table}[t]
\begin{center}
\caption{\UseMacro{TCap-dataset-edits-stats}}
\vspace{-8pt}
\begin{tabular}{l  l | r  r  r }
\toprule
 & 
 & \textbf{\UseMacro{THead-train}}
 & \textbf{\UseMacro{THead-valid}}
 & \textbf{\UseMacro{THead-test}}
\\
\midrule
\multicolumn{2}{l|}{\UseMacro{THead-count}}
% \UseMacro{THead-count}
 & \UseMacro{ds-train-count}
 & \UseMacro{ds-valid-count}
 & \UseMacro{ds-test-count}
 \\
 \midrule
\multirow{5}{*}{Java}
& \UseMacro{THead-mean-old-method-size}
 & \UseMacro{train-java-mean-old-method-size}
 & \UseMacro{valid-java-mean-old-method-size}
 & \UseMacro{test-java-mean-old-method-size}
\\
&\UseMacro{THead-mean-new-method-size}
 & \UseMacro{train-java-mean-new-method-size}
 & \UseMacro{valid-java-mean-new-method-size}
 & \UseMacro{test-java-mean-new-method-size}
\\
&\UseMacro{THead-mean-edit-actions}
 & \UseMacro{train-java-mean-edit-actions}
 & \UseMacro{valid-java-mean-edit-actions}
 & \UseMacro{test-java-mean-edit-actions}
\\
% &\UseMacro{THead-mean-edit-tokens}
%  & \UseMacro{train-java-mean-edit-tokens}
%  & \UseMacro{valid-java-mean-edit-tokens}
%  & \UseMacro{test-java-mean-edit-tokens}
% \\
&\UseMacro{THead-mean-add-tokens}
 & \UseMacro{train-java-mean-add-tokens}
 & \UseMacro{valid-java-mean-add-tokens}
 & \UseMacro{test-java-mean-add-tokens}
\\
&\UseMacro{THead-mean-del-tokens}
 & \UseMacro{train-java-mean-del-tokens}
 & \UseMacro{valid-java-mean-del-tokens}
 & \UseMacro{test-java-mean-del-tokens}
\\
% &\UseMacro{THead-mean-edit-lines}
%  & \UseMacro{train-java-mean-edit-lines}
%  & \UseMacro{valid-java-mean-edit-lines}
%  & \UseMacro{test-java-mean-edit-lines}
% \\
\midrule
\multirow{5}{*}{C\#}
&\UseMacro{THead-mean-old-method-size}
 & \UseMacro{train-cs-mean-old-method-size}
 & \UseMacro{valid-cs-mean-old-method-size}
 & \UseMacro{test-cs-mean-old-method-size}
\\
&\UseMacro{THead-mean-new-method-size}
 & \UseMacro{train-cs-mean-new-method-size}
 & \UseMacro{valid-cs-mean-new-method-size}
 & \UseMacro{test-cs-mean-new-method-size}
\\
&\UseMacro{THead-mean-edit-actions}
 & \UseMacro{train-cs-mean-edit-actions}
 & \UseMacro{valid-cs-mean-edit-actions}
 & \UseMacro{test-cs-mean-edit-actions}
\\
% &\UseMacro{THead-mean-edit-tokens}
%  & \UseMacro{train-cs-mean-edit-tokens}
%  & \UseMacro{valid-cs-mean-edit-tokens}
%  & \UseMacro{test-cs-mean-edit-tokens}
% \\
&\UseMacro{THead-mean-add-tokens}
 & \UseMacro{train-cs-mean-add-tokens}
 & \UseMacro{valid-cs-mean-add-tokens}
 & \UseMacro{test-cs-mean-add-tokens}
\\
&\UseMacro{THead-mean-del-tokens}
 & \UseMacro{train-cs-mean-del-tokens}
 & \UseMacro{valid-cs-mean-del-tokens}
 & \UseMacro{test-cs-mean-del-tokens}
\\
% &\UseMacro{THead-mean-edit-lines}
%  & \UseMacro{train-cs-mean-edit-lines}
%  & \UseMacro{valid-cs-mean-edit-lines}
%  & \UseMacro{test-cs-mean-edit-lines}
% \\
\bottomrule
\end{tabular}
\vspace{\UseMacro{TVspace-dataset-edits-stats}}
\end{center}
\end{table}


==> tables/table-edits-sequence.tex <==
%% Manually created by Jiyang

\newcommand{\specialtwocell}[2][c]{%
  \begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}

\newcommand{\specialthreecell}[2][c]{%
  \begin{tabular}[#1]{@{}l@{}l@{}}#2\end{tabular}}

\begin{small}
\begin{table}[t]
\begin{center}
\caption{\UseMacro{TCap-edits-map}}
\vspace{-8pt}
\begin{tabular}{l l l}
    \toprule
    \textbf{Edit}
    & \textbf{\Concise}
    & \textbf{\Unambig}
    \\
    \midrule
    \multirow{2}{*}{Insertion}
    & \multirow{2}{*}{\texttt{<Insert>}}
    &
    \specialtwocell[t]{\texttt{<ReplaceKeepBefore>}\\ \texttt{<ReplaceKeepAfter>}}
    \\
    \midrule
    % Deletions
    \multirow{3}{*}{Deletion}
    & \multirow{3}{*}{\texttt{<Delete>}}
    & %\texttt{<Delete>}, \texttt{<ReplaceNewKeepAfter>}, \texttt{<ReplaceNewKeepBefore>}
    \specialthreecell[t]{\texttt{<Delete>} \\ \texttt{<ReplaceKeepBefore>}\\ \texttt{<ReplaceKeepAfter>}}
    \\
    \midrule
    \multirow{3}{*}{Replacement}
    & \multirow{3}{*}{\texttt{<Replace>}}
    & \specialthreecell[t]{\texttt{<Replace>} \\ \texttt{<ReplaceKeepBefore>}\\ \texttt{<ReplaceKeepAfter>}}
    \\
    \bottomrule
\end{tabular}
\vspace{\UseMacro{TVspace-edits-map}}
\end{center}
\end{table}
\end{small}


==> tables/table-java2cs-ag-translation-models-results.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}[t]
\begin{center}
\caption{\UseMacro{TCap-java2cs-ag-translation-models-results}}
\vspace{-7pt}
\begin{tabular}{l | c  c  c  c }
\toprule
\textbf{\UseMacro{THead-models}}
 & \textbf{\UseMacro{THead-Acc-top-1}}
 & \textbf{\UseMacro{THead-BLEU}}
 & \textbf{\UseMacro{THead-CodeBLEU}}
\\
\midrule
\UseMacro{THead-translation-CodeT5}
 & \UseMacro{res-java2cs-ag-translation-CodeT5-Acc-top-1}
 & \UseMacro{res-java2cs-ag-translation-CodeT5-BLEU}
 & \UseMacro{res-java2cs-ag-translation-CodeT5-CodeBLEU}
\\
\UseMacro{THead-update-CodeT5}
 & \textbf{\UseMacro{res-java2cs-ag-update-CodeT5-Acc-top-1}}
 & \textbf{\UseMacro{res-java2cs-ag-update-CodeT5-BLEU}}
 & \textbf{\UseMacro{res-java2cs-ag-update-CodeT5-CodeBLEU}}
\\
\bottomrule
\end{tabular}
\label{tab:java2cs-agtranslation-results}
\end{center}
\end{table*}


==> tables/table-java2cs-clean-translation-models-results.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}[t]
\begin{center}
\caption{\UseMacro{TCap-java2cs-clean-translation-models-results}}
\begin{tabular}{l | c  c  c  c }
\toprule
\textbf{\UseMacro{THead-models}}
 & \textbf{\UseMacro{THead-Acc-top-1}}
 & \textbf{\UseMacro{THead-BLEU}}
 & \textbf{\UseMacro{THead-CodeBLEU}}
\\
\midrule
\UseMacro{THead-translation-CodeT5}
 & \UseMacro{res-java2cs-clean-translation-CodeT5-Acc-top-1}
 & \UseMacro{res-java2cs-clean-translation-CodeT5-BLEU}
 & \UseMacro{res-java2cs-clean-translation-CodeT5-CodeBLEU}
\\
\UseMacro{THead-translation-CodeT5-ag}
 & \UseMacro{res-java2cs-clean-translation-CodeT5-ag-Acc-top-1}
 & \UseMacro{res-java2cs-clean-translation-CodeT5-ag-BLEU}
 & \UseMacro{res-java2cs-clean-translation-CodeT5-ag-CodeBLEU}
\\
% \UseMacro{THead-translation-CoditT5}
%  & \UseMacro{res-java2cs-clean-translation-CoditT5-Acc-top-1}
%  & \UseMacro{res-java2cs-clean-translation-CoditT5-BLEU}
%  & \UseMacro{res-java2cs-clean-translation-CoditT5-CodeBLEU}
% \\
\UseMacro{THead-update-CodeT5}
 & \UseMacro{res-java2cs-clean-update-CodeT5-Acc-top-1}
 & \UseMacro{res-java2cs-clean-update-CodeT5-BLEU}
 & \UseMacro{res-java2cs-clean-update-CodeT5-CodeBLEU}
\\
\UseMacro{THead-update-CodeT5-ag}
 & \textbf{\UseMacro{res-java2cs-clean-update-CodeT5-ag-Acc-top-1}}
 & \textbf{\UseMacro{res-java2cs-clean-update-CodeT5-ag-BLEU}}
 & \textbf{\UseMacro{res-java2cs-clean-update-CodeT5-ag-CodeBLEU}}
\\
\UseMacro{THead-align-CoditT5}
 & \UseMacro{res-java2cs-clean-align-CoditT5-Acc-top-1}
 & \UseMacro{res-java2cs-clean-align-CoditT5-BLEU}
 & \UseMacro{res-java2cs-clean-align-CoditT5-CodeBLEU}
\\
\UseMacro{THead-align-CoditT5-ag}
 & \UseMacro{res-java2cs-clean-align-CoditT5-ag-Acc-top-1}
 & \UseMacro{res-java2cs-clean-align-CoditT5-ag-BLEU}
 & \UseMacro{res-java2cs-clean-align-CoditT5-ag-CodeBLEU}
\\
\bottomrule
\end{tabular}
\label{tab:java2cs-cleantranslation-results}
\end{center}
\end{table*}


==> tables/table-java2cs-cp-translation-models-results.tex <==
%% Automatically generated by: Table.py make_table_results

\begin{table*}[t]
\begin{center}
\caption{\UseMacro{TCap-java2cs-cp-translation-models-results}}
\vspace{-8pt}
\begin{tabular}{l | c  c  c  c  c  c }
\toprule
\textbf{\UseMacro{THead-models}}
 & \textbf{\UseMacro{THead-Acc-top-1}}
 & \textbf{\UseMacro{THead-BLEU}}
 & \textbf{\UseMacro{THead-CodeBLEU}}
 & \textbf{\UseMacro{THead-SARI}}
 & \textbf{\UseMacro{THead-GLEU}}
\\
\midrule
\UseMacro{THead-copy}
 & \UseMacro{res-java2cs-cp-copy-Acc-top-1}
 & \UseMacro{res-java2cs-cp-copy-BLEU}$^{\alpha}$
 & \UseMacro{res-java2cs-cp-copy-CodeBLEU}
 & \UseMacro{res-java2cs-cp-copy-SARI}
 & \UseMacro{res-java2cs-cp-copy-GLEU}
\\
\UseMacro{THead-CopyEdits}
 & \UseMacro{res-java2cs-cp-CopyEdits-Acc-top-1}
 & \UseMacro{res-java2cs-cp-CopyEdits-BLEU}
 & \UseMacro{res-java2cs-cp-CopyEdits-CodeBLEU}
 & \UseMacro{res-java2cs-cp-CopyEdits-SARI}
 & \UseMacro{res-java2cs-cp-CopyEdits-GLEU}
\\
\midrule
\UseMacro{THead-translation-CodeT5}
 & \UseMacro{res-java2cs-cp-translation-CodeT5-Acc-top-1}
 & \UseMacro{res-java2cs-cp-translation-CodeT5-BLEU}
 & \UseMacro{res-java2cs-cp-translation-CodeT5-CodeBLEU}
 & \UseMacro{res-java2cs-cp-translation-CodeT5-SARI}
 & \UseMacro{res-java2cs-cp-translation-CodeT5-GLEU}
\\
\UseMacro{THead-update-CodeT5}
 & \UseMacro{res-java2cs-cp-update-CodeT5-Acc-top-1}
 & \UseMacro{res-java2cs-cp-update-CodeT5-BLEU}$^{\alpha}$
 & \UseMacro{res-java2cs-cp-update-CodeT5-CodeBLEU}
 & \UseMacro{res-java2cs-cp-update-CodeT5-SARI}
 & \UseMacro{res-java2cs-cp-update-CodeT5-GLEU}
\\
\UseMacro{THead-CoditT5}
 & \UseMacro{res-java2cs-cp-CoditT5-Acc-top-1}
 & \UseMacro{res-java2cs-cp-CoditT5-BLEU}
 & \UseMacro{res-java2cs-cp-CoditT5-CodeBLEU}
 & \UseMacro{res-java2cs-cp-CoditT5-SARI}
 & \UseMacro{res-java2cs-cp-CoditT5-GLEU}
\\
\UseMacro{THead-chatgpt3.5-zero-shot}
 & \UseMacro{res-java2cs-cp-chatgpt3.5-zero-shot-Acc-top-1}
 & \UseMacro{res-java2cs-cp-chatgpt3.5-zero-shot-BLEU}
 & \UseMacro{res-java2cs-cp-chatgpt3.5-zero-shot-CodeBLEU}
 & \UseMacro{res-java2cs-cp-chatgpt3.5-zero-shot-SARI}
 & \UseMacro{res-java2cs-cp-chatgpt3.5-zero-shot-GLEU}
\\
\midrule
\UseMacro{THead-metaEdits}
 & \UseMacro{res-java2cs-cp-metaEdits-Acc-top-1}
 & \UseMacro{res-java2cs-cp-metaEdits-BLEU}$^{\beta}$
 & \UseMacro{res-java2cs-cp-metaEdits-CodeBLEU}
 & \UseMacro{res-java2cs-cp-metaEdits-SARI}
 & \UseMacro{res-java2cs-cp-metaEdits-GLEU}$^{\chi}$
\\
\UseMacro{THead-edit-translation}
 & \UseMacro{res-java2cs-cp-edit-translation-Acc-top-1}
 & \UseMacro{res-java2cs-cp-edit-translation-BLEU}$^{\beta}$
 & \UseMacro{res-java2cs-cp-edit-translation-CodeBLEU}
 & \UseMacro{res-java2cs-cp-edit-translation-SARI}
 & \UseMacro{res-java2cs-cp-edit-translation-GLEU}$^{\chi}$
\\
\midrule
\UseMacro{THead-hybrid}
 & \textbf{\UseMacro{res-java2cs-cp-hybrid-Acc-top-1}}
 & \textbf{\UseMacro{res-java2cs-cp-hybrid-BLEU}}
 & \textbf{\UseMacro{res-java2cs-cp-hybrid-CodeBLEU}}
 & \textbf{\UseMacro{res-java2cs-cp-hybrid-SARI}}
 & \textbf{\UseMacro{res-java2cs-cp-hybrid-GLEU}}
\\
\bottomrule
\end{tabular}
\label{tab:java2cs-cp-translation-results}
\end{center}
\end{table*}

==> tables/table-java2cs-new-test-translation-models-results.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}[t]
\begin{center}
\caption{\UseMacro{TCap-java2cs-new-test-translation-models-results}}
\begin{tabular}{l | c  c  c  c  c }
\toprule
\textbf{\UseMacro{THead-models}}
 & \textbf{\UseMacro{THead-Acc-top-1}}
 & \textbf{\UseMacro{THead-BLEU}}
 & \textbf{\UseMacro{THead-CodeBLEU}}
 & \textbf{\UseMacro{THead-ngram_match_score}}
\\
\midrule
\UseMacro{THead-copy}
 & \UseMacro{res-java2cs-new-test-copy-Acc-top-1}
 & \UseMacro{res-java2cs-new-test-copy-BLEU}
 & \UseMacro{res-java2cs-new-test-copy-CodeBLEU}
 & \UseMacro{res-java2cs-new-test-copy-ngram_match_score}
\\
\UseMacro{THead-CopyEdits}
 & \UseMacro{res-java2cs-new-test-CopyEdits-Acc-top-1}
 & \UseMacro{res-java2cs-new-test-CopyEdits-BLEU}
 & \UseMacro{res-java2cs-new-test-CopyEdits-CodeBLEU}
 & \UseMacro{res-java2cs-new-test-CopyEdits-ngram_match_score}
\\
\midrule
\UseMacro{THead-translation-CodeT5}
 & \UseMacro{res-java2cs-new-test-translation-CodeT5-Acc-top-1}
 & \UseMacro{res-java2cs-new-test-translation-CodeT5-BLEU}
 & \UseMacro{res-java2cs-new-test-translation-CodeT5-CodeBLEU}
 & \UseMacro{res-java2cs-new-test-translation-CodeT5-ngram_match_score}
\\
\UseMacro{THead-CoditT5}
 & \textbf{\UseMacro{res-java2cs-new-test-CoditT5-Acc-top-1}}
 & \textbf{\UseMacro{res-java2cs-new-test-CoditT5-BLEU}}
 & \UseMacro{res-java2cs-new-test-CoditT5-CodeBLEU}
 & \UseMacro{res-java2cs-new-test-CoditT5-ngram_match_score}
\\
\UseMacro{THead-update-CodeT5}
 & \UseMacro{res-java2cs-new-test-update-CodeT5-Acc-top-1}
 & \UseMacro{res-java2cs-new-test-update-CodeT5-BLEU}
 & \textbf{\UseMacro{res-java2cs-new-test-update-CodeT5-CodeBLEU}}
 & \UseMacro{res-java2cs-new-test-update-CodeT5-ngram_match_score}
\\
\UseMacro{THead-metaEdits}
 & \UseMacro{res-java2cs-new-test-metaEdits-Acc-top-1}
 & \UseMacro{res-java2cs-new-test-metaEdits-BLEU}
 & \UseMacro{res-java2cs-new-test-metaEdits-CodeBLEU}
 & \UseMacro{res-java2cs-new-test-metaEdits-ngram_match_score}
\\
\UseMacro{THead-edit-translation}
 & \UseMacro{res-java2cs-new-test-edit-translation-Acc-top-1}
 & \UseMacro{res-java2cs-new-test-edit-translation-BLEU}
 & \UseMacro{res-java2cs-new-test-edit-translation-CodeBLEU}
 & \textbf{\UseMacro{res-java2cs-new-test-edit-translation-ngram_match_score}}
\\
\bottomrule
\end{tabular}
\label{tab:java2cs-new-testtranslation-results}
\end{center}
\end{table*}


==> tables/table-java2cs-synthetic-dataset.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}
\begin{center}
\caption{\UseMacro{TCap-java2cs-synthetic-dataset}}
\begin{tabular}{l | r }
\toprule
\textbf{\UseMacro{THead-project}}
 & \textbf{\UseMacro{THead-count}}
\\
\midrule
antlr-antlr4
 & \UseMacro{ds-antlr-antlr4-count}
\\
apache-lucene
 & \UseMacro{ds-apache-lucene-count}
\\
apache-poi
 & \UseMacro{ds-apache-poi-count}
\\
eclipse-jgit
 & \UseMacro{ds-eclipse-jgit-count}
\\
formicary-fpml-toolkit-java
 & \UseMacro{ds-formicary-fpml-toolkit-java-count}
\\
itext-itext7
 & \UseMacro{ds-itext-itext7-count}
\\
quartz-scheduler-quartz
 & \UseMacro{ds-quartz-scheduler-quartz-count}
\\
terabyte-jgit
 & \UseMacro{ds-terabyte-jgit-count}
\\
total
 & \UseMacro{ds-total-count}
\\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> tables/table-java2cs-translation-dataset.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}
\begin{center}
\caption{\UseMacro{TCap-java2cs-translation-dataset}}
\vspace{-10pt}
\begin{tabular}{l | r  r  r  r  r  r }
\toprule
 
 & \textbf{\UseMacro{THead-train}}
 & \textbf{\UseMacro{THead-valid}}
 & \textbf{\UseMacro{THead-test}}
%  & \textbf{\UseMacro{THead-cleaned-test}}
%  & \textbf{\UseMacro{THead-augment}}
%  & \textbf{\UseMacro{THead-semi}}
\\
\midrule
\UseMacro{THead-count}
 & \UseMacro{ds-train-count}
 & \UseMacro{ds-valid-count}
 & \UseMacro{ds-test-count}
%  & \UseMacro{ds-cleaned-test-count}
%  & \UseMacro{ds-augment-count}
%  & \UseMacro{ds-semi-count}
\\
\UseMacro{THead-cs-edit-distance-mean}
 & \UseMacro{ds-train-cs-edit-distance-mean}
 & \UseMacro{ds-valid-cs-edit-distance-mean}
 & \UseMacro{ds-test-cs-edit-distance-mean}
%  & \UseMacro{ds-cleaned-test-cs-edit-distance-mean}
%  & N/A
%  & \UseMacro{ds-semi-cs-edit-distance-mean}
\\
\UseMacro{THead-java-edit-distance-mean}
 & \UseMacro{ds-train-java-edit-distance-mean}
 & \UseMacro{ds-valid-java-edit-distance-mean}
 & \UseMacro{ds-test-java-edit-distance-mean}
%  & \UseMacro{ds-cleaned-test-java-edit-distance-mean}
%  & N/A
%  & \UseMacro{ds-semi-java-edit-distance-mean}
\\
\bottomrule
\end{tabular}
\label{tab: dataset-split-stats}
\end{center}
\end{table*}


==> tables/table-java2cs-translation-models-results.tex <==
%% Automatically generated by: Table.py make_table_results

\begin{table*}[t]
\begin{center}
\caption{\UseMacro{TCap-java2cs-translation-models-results}}
\vspace{-8pt}
\begin{tabular}{l | c  c  c  c  c  c }
\toprule
\textbf{\UseMacro{THead-models}}
 & \textbf{\UseMacro{THead-Acc-top-1}}
 & \textbf{\UseMacro{THead-BLEU}}
 & \textbf{\UseMacro{THead-CodeBLEU}}
 & \textbf{\UseMacro{THead-SARI}}
 & \textbf{\UseMacro{THead-GLEU}}
\\
\midrule
\UseMacro{THead-copy}
 & \UseMacro{res-java2cs-copy-Acc-top-1}
 & \UseMacro{res-java2cs-copy-BLEU}
 & \UseMacro{res-java2cs-copy-CodeBLEU}
 & \UseMacro{res-java2cs-copy-SARI}
 & \UseMacro{res-java2cs-copy-GLEU}
\\
\UseMacro{THead-CopyEdits}
 & \UseMacro{res-java2cs-CopyEdits-Acc-top-1}$^{\beta}$
 & \UseMacro{res-java2cs-CopyEdits-BLEU}$^{\alpha}$$^{\chi}$
 & \UseMacro{res-java2cs-CopyEdits-CodeBLEU}
 & \UseMacro{res-java2cs-CopyEdits-SARI}
 & \UseMacro{res-java2cs-CopyEdits-GLEU}
\\
\midrule
\UseMacro{THead-translation-CodeT5}
 & \UseMacro{res-java2cs-translation-CodeT5-Acc-top-1}$^{\beta}$
 & \UseMacro{res-java2cs-translation-CodeT5-BLEU}
 & \UseMacro{res-java2cs-translation-CodeT5-CodeBLEU}
 & \UseMacro{res-java2cs-translation-CodeT5-SARI}
 & \UseMacro{res-java2cs-translation-CodeT5-GLEU}
\\
\UseMacro{THead-update-CodeT5}
 & \UseMacro{res-java2cs-update-CodeT5-Acc-top-1}$^{\epsilon}$
 & \UseMacro{res-java2cs-update-CodeT5-BLEU}$^{\chi}$$^{\eta}$
 & \UseMacro{res-java2cs-update-CodeT5-CodeBLEU}
 & \UseMacro{res-java2cs-update-CodeT5-SARI}
 & \UseMacro{res-java2cs-update-CodeT5-GLEU}
\\
\UseMacro{THead-CoditT5}
 & \UseMacro{res-java2cs-CoditT5-Acc-top-1}$^{\epsilon}$
 & \UseMacro{res-java2cs-CoditT5-BLEU}$^{\alpha}$$^{\eta}$
 & \UseMacro{res-java2cs-CoditT5-CodeBLEU}
 & \UseMacro{res-java2cs-CoditT5-SARI}
 & \UseMacro{res-java2cs-CoditT5-GLEU}
\\
\UseMacro{THead-codex}
 & \UseMacro{res-java2cs-codex-Acc-top-1}
 & \UseMacro{res-java2cs-codex-BLEU}
 & \UseMacro{res-java2cs-codex-CodeBLEU}
 & \UseMacro{res-java2cs-codex-SARI}
 & \UseMacro{res-java2cs-codex-GLEU}
\\
\UseMacro{THead-chatgpt3.5-zero-shot}
 & \UseMacro{res-java2cs-chatgpt3.5-zero-shot-Acc-top-1}
 & \UseMacro{res-java2cs-chatgpt3.5-zero-shot-BLEU}
 & \UseMacro{res-java2cs-chatgpt3.5-zero-shot-CodeBLEU}
 & \UseMacro{res-java2cs-chatgpt3.5-zero-shot-SARI}
 & \UseMacro{res-java2cs-chatgpt3.5-zero-shot-GLEU}
\\
\midrule
\UseMacro{THead-metaEdits}
 & \UseMacro{res-java2cs-metaEdits-Acc-top-1}
 & \UseMacro{res-java2cs-metaEdits-BLEU}
 & \UseMacro{res-java2cs-metaEdits-CodeBLEU}
 & \UseMacro{res-java2cs-metaEdits-SARI}
 & \UseMacro{res-java2cs-metaEdits-GLEU}
\\
\UseMacro{THead-edit-translation}
 & \UseMacro{res-java2cs-edit-translation-Acc-top-1}
 & \UseMacro{res-java2cs-edit-translation-BLEU}
 & \UseMacro{res-java2cs-edit-translation-CodeBLEU}
 & \textbf{\UseMacro{res-java2cs-edit-translation-SARI}}$^{\delta}$
 & \UseMacro{res-java2cs-edit-translation-GLEU}
\\
\midrule
\UseMacro{THead-hybrid}
 & \textbf{\UseMacro{res-java2cs-hybrid-Acc-top-1}}
 & \textbf{\UseMacro{res-java2cs-hybrid-BLEU}}
 & \textbf{\UseMacro{res-java2cs-hybrid-CodeBLEU}}
 & \UseMacro{res-java2cs-hybrid-SARI}$^{\delta}$
 & \textbf{\UseMacro{res-java2cs-hybrid-GLEU}}
\\
\bottomrule
\end{tabular}
\label{tab:java2cstranslation-results}
\end{center}
\end{table*}

==> tables/table-real-world-dataset-split.tex <==

%% Automatically generated by pyutil.latex 

\begin{table*}[t]
\begin{center}
\caption{\UseMacro{TCap-real-world-dataset-split}}

\begin{tabular}{l | r  r  r  r  r }
\toprule
\textbf{\UseMacro{THead-project}}
 & \textbf{\UseMacro{THead-count}}
 & \textbf{\UseMacro{THead-train-commit}}
 & \textbf{\UseMacro{THead-valid-commit}}
 & \textbf{\UseMacro{THead-test-commit}}
\\
\midrule
antlr-antlr4
 & \UseMacro{antlr-antlr4-count}
 & \UseMacro{antlr-antlr4-cs-train-commit}
 & \UseMacro{antlr-antlr4-cs-valid-commit}
 & \UseMacro{antlr-antlr4-cs-test-commit}
\\
apache-lucene
 & \UseMacro{apache-lucene-count}
 & \UseMacro{apache-lucene-cs-train-commit}
 & \UseMacro{apache-lucene-cs-valid-commit}
 & \UseMacro{apache-lucene-cs-test-commit}
\\
apache-poi
 & \UseMacro{apache-poi-count}
 & \UseMacro{apache-poi-cs-train-commit}
 & \UseMacro{apache-poi-cs-valid-commit}
 & \UseMacro{apache-poi-cs-test-commit}
\\
itext-itext7
 & \UseMacro{itext-itext7-count}
 & \UseMacro{itext-itext7-cs-train-commit}
 & \UseMacro{itext-itext7-cs-valid-commit}
 & \UseMacro{itext-itext7-cs-test-commit}
\\
formicary-fpml-toolkit-java
 & \UseMacro{formicary-fpml-toolkit-java-count}
 & \UseMacro{formicary-fpml-toolkit-java-cs-train-commit}
 & \UseMacro{formicary-fpml-toolkit-java-cs-valid-commit}
 & \UseMacro{formicary-fpml-toolkit-java-cs-test-commit}
\\
eclipse-jgit
 & \UseMacro{eclipse-jgit-count}
 & \UseMacro{eclipse-jgit-cs-train-commit}
 & \UseMacro{eclipse-jgit-cs-valid-commit}
 & \UseMacro{eclipse-jgit-cs-test-commit}
\\
quartz-scheduler-quartz
 & \UseMacro{quartz-scheduler-quartz-count}
 & \UseMacro{quartz-scheduler-quartz-cs-train-commit}
 & \UseMacro{quartz-scheduler-quartz-cs-valid-commit}
 & \UseMacro{quartz-scheduler-quartz-cs-test-commit}
\\
terabyte-jgit
 & \UseMacro{terabyte-jgit-count}
 & \UseMacro{terabyte-jgit-cs-train-commit}
 & \UseMacro{terabyte-jgit-cs-valid-commit}
 & \UseMacro{terabyte-jgit-cs-test-commit}
\\
\bottomrule
\end{tabular}
\end{center}
\end{table*}


==> tables/table-real-world-dataset.tex <==

%% Automatically generated by pyutil.latex 

\begin{table}[t]
\begin{center}
\caption{\UseMacro{TCap-real-world-dataset-stats}}
\vspace{-8pt}
\begin{small}
\begin{tabular}{l l  r }
\toprule
\textbf{\UseMacro{THead-java-project}}
 & \textbf{\UseMacro{THead-cs-project}}
 & \textbf{\UseMacro{THead-count}}
\\
\midrule
antlr/antlr4
& tunnelvisionlabs/antlr4cs
 & \UseMacro{antlr-antlr4-count}
\\
apache/lucene
& apache/lucenenet
 & \UseMacro{apache-lucene-count}
\\
apache/poi
&nissl-lab/npoi
 & \UseMacro{apache-poi-count}
\\
eclipse/jgit
& mono/ngit
 & \UseMacro{eclipse-jgit-count}
\\
formicary/fpml-toolkit-java
& formicary/fpml-toolkit-csharp
 & \UseMacro{formicary-fpml-toolkit-java-count}
\\
itext/itext7
& itext/itext7-dotnet
 & \UseMacro{itext-itext7-count}
 \\
quartz-scheduler/quartz
& quartznet/quartznet
 & \UseMacro{quartz-scheduler-quartz-count}
\\
terabyte/jgit
& mono/ngit
 & \UseMacro{terabyte-jgit-count}
\\
\midrule
\textbf{SUM}
&
& \Datasize\\
\bottomrule
\end{tabular}
\vspace{\UseMacro{TVspace-real-world-dataset-stats}}
\end{small}
\end{center}
\end{table}

